Trustworthy and Explainable Decision-Making for Workforce allocation

In industrial contexts, effective workforce allocation is crucial for operational efficiency. This paper presents an ongoing project focused on developing a decision-making tool designed for workforce allocation, emphasising the explainability to enhance its trustworthiness. Our objective is to create a system that not only optimises the allocation of teams to scheduled tasks but also provides clear, understandable explanations for its decisions, particularly in cases where the problem is infeasible. By incorporating human-in-the-loop mechanisms, the tool aims to enhance user trust and facilitate interactive conflict resolution. We implemented our approach on a prototype tool/digital demonstrator intended to be evaluated on a real industrial scenario both in terms of performance and user acceptability.

==> table_optim.tex <==
\begin{table}
\caption{Mean computation by different lengths of instance and configurations, with ortools-cpsat and 6 process}
\label{tab:grouped_df}
\begin{tabular}{rrrrrrrr}
\toprule
length & red\_overlap & symm\_used & t\_init (s) & t\_solve (s) & t\_total (s) & \% optimal \\
\midrule
6 & False & False & 0.03 & 0.06 & 0.09 & 100\% \\
6 & False & True & 0.03 & 0.18 & 0.21 & 100\% \\
6 & True & False & 0.06 & 0.06 & 0.12 & 100\% \\
6 & True & True & 0.06 & 0.17 & 0.24 & 100\% \\
8 & False & False & 0.04 & 0.08 & 0.12 & 100\% \\
8 & False & True & 0.04 & 0.19 & 0.23 & 100\% \\
8 & True & False & 0.08 & 0.09 & 0.17 & 100\% \\
8 & True & True & 0.08 & 0.22 & 0.30 & 100\% \\
24 & False & False & 0.12 & 0.29 & 0.41 & 100\% \\
24 & False & True & 0.12 & 0.57 & 0.69 & 100\% \\
24 & True & False & 0.34 & 0.32 & 0.66 & 100\% \\
24 & True & True & 0.33 & 0.72 & 1.06 & 100\% \\
\bottomrule
\end{tabular}
\label{optim-res}
\end{table}


==> table_optim_1proc.tex <==
\begin{table}
\caption{Mean computation by different lengths of instance and configurations
running ortools-cpsat with 1 process}
\label{tab:grouped_df}
\begin{tabular}{rrrrrrrr}
\toprule
length & red\_overlap & symm\_used & t\_init (s) & t\_solve (s) & t\_total (s) & \% optimal \\
\midrule
6 & False & False & 0.03 & 12.21 & 12.24 & 45\% \\
6 & False & True & 0.03 & 2.01 & 2.04 & 95\% \\
6 & True & False & 0.06 & 10.98 & 11.04 & 45\% \\
6 & True & True & 0.06 & 2.03 & 2.09 & 95\% \\
8 & False & False & 0.04 & 13.13 & 13.17 & 45\% \\
8 & False & True & 0.04 & 2.93 & 2.97 & 95\% \\
8 & True & False & 0.08 & 12.99 & 13.06 & 40\% \\
8 & True & True & 0.08 & 2.44 & 2.52 & 95\% \\
24 & False & False & 0.12 & 14.64 & 14.76 & 30\% \\
24 & False & True & 0.12 & 5.54 & 5.66 & 85\% \\
24 & True & False & 0.33 & 14.61 & 14.94 & 30\% \\
24 & True & True & 0.33 & 5.06 & 5.39 & 85\% \\
\bottomrule
\end{tabular}
\label{results-1proc}
\end{table}

